High flexoelectric constants in Janus transition-metal dichalcogenides

Due to their combination of mechanical stiffness and flexibility, two-dimensional (2D) materials have received significant interest as potential electromechanical materials. Flexoelectricity is an electromechanical coupling between strain gradient and polarization. Unlike piezoelectricity, which exists only in non-centrosymmetric materials, flexoelectricity theoretically exists in all dielectric materials. However, most work on the electromechanical energy conversion potential of 2D materials has focused on their piezoelectric, and not flexoelectric behavior and properties. In the present work, we demonstrate that the intrinsic structural asymmetry present in monolayer Janus transition metal dichalcogenides (TMDCs) enables significant flexoelectric properties. We report these flexoelectric properties using a recently developed charge-dipole model that couples with classical molecular dynamics simulations. By employing a prescribed bending deformation, we directly calculate the flexoelectric constants while eliminating the piezoelectric contribution to the polarization. We find that the flexoelectric response of a Janus TMDC is positively correlated to its initial degree of asymmetry, which contributes to stronger $\sigma-\sigma$ interactions as the initial degree of asymmetry rises. In addition, the high transfer of charge across atoms in Janus TMDCs leads to larger electric fields due to $\pi-\sigma$ coupling. These enhanced $\sigma-\sigma$ and $\pi-\sigma$ interactions are found to cause the flexoelectric coefficients of the Janus TMDCs to be several times higher than traditional TMDCs such as MoS$_{2}$, whose flexoelectric constant is already ten times larger than graphene.

==> extra.tex <==
%\noindent Flexoelectricity is a electromechanical phenomenon describes the coupling between strain gradient and induced electrical polarization. Unlike piezoelectricity, which exists only in the material with non-centrosymmetric crystal structure, flexoelectricity prevails in all dielectric material. \bh{Janus monolayer transition-metal dichalcogenides (JTMDCs) recently attract significant interest due to their remarkable electromechanical properties and flexibility. This sentence we may have to remove or rewrite} In this study, the molecular dynamics equipped with the charge-dipole model is employed to investigates the flexoelectric response in Janus TMDCs.  A specific loading scheme is adopted in this study for accomplishing the direct measurement of flexoelectric response in Janus TMDCs without the intervention of the piezoelectricity. It is found that the flexoelectric response of a Janus TMDC is positive correlated to its initial degree of asymmetry, which contribute to a stronger $\sigma-\sigma$ interaction as the initial degree of asymmetry rises. Due to the strong $\sigma-\sigma$ interaction, the flexoelectric of coefficients of the Janus TMDCs are observed several times higher than traditional TMDC: such as MoS2, which already has the flexoelectric coefficient ten times larger than Graphene. 
%%%%%%%%%%%%%%%%%%
%\section{Introduction}
%\label{sec:introduction}
%\noindent Energy harvester \cite{ikeda1996fundamentals,heywang2008piezoelectricity} utilizing the piezoelectric effect for converting mechanical energy into electrical energy has been developed for several decades. While the piezoelectric effect is well understood and utilized, another type of electromechanical coupling phenomenon: flexoelectricitiy, has recently attracted significant attentions \cite{ma2002flexoelectric,harden2006giant,hong2010flexoelectricity,krichen2016flexoelectricity}, for the reason that the flexoelectric effect prevails in all materials regardless of their crystal structure, which piezoelectric effect is depended on. The mechanical induced electrical polarization in a dielectric material is governed by \cite{Tagantsev1986}
%\begin{equation}
%P^{\alpha} = d^{\alpha \beta \gamma}\epsilon^{\beta \gamma} + \mu^{\alpha \beta \gamma \delta}\frac{\partial\epsilon^{\gamma \delta}}{\partial x_{\beta}},
%\label{eq:polarization}
%\end{equation}
%where $d^{\alpha \beta \gamma}$ and $\mu^{\alpha \beta \gamma \delta}$ represents the piezoelectric and flexoelectric coefficient, respectively. Accordingly, the $\epsilon^{\beta \gamma}$ and  $\frac{\partial\epsilon^{\gamma \delta}}{\partial x_{\beta}}$ is the strain and strain gradient, respectively. $\alpha$, $\beta$, $\gamma$ and $\delta$ represent the axial components of the coordinate system.\\
%\noindent Two-dimensional materials \cite{Wang2015observattion,Song2017piezo,Zheng2017hexagonal,Zelisko2014anomalous,blonsky2015ab} including Janus TMDCs \cite{dong2017large} have exhibited outstanding electromechanical properties. However the aforementioned studies mainly focus on the piezoelectric effect of the 2D materials. In the meantime, Majdoub, et. al. \cite{majdoub2008enhanced} demonstrated that the flexoelectric effect is size-dependent, which yields a stronger electromechanical coupling at smaller scale, hence presents a great opportunity for low dimension 2D material, such as Janus TMDCs, as the next generation energy harvester thanks to their intrinsic small scale. \\
%\noindent Contrast to the extensive studies on the piezoelectric effect in 2d material, few studies on flexoelectricity in 2D materials are conducted. For instance, A Density function theory (DFT) study revealed a linear relationship between the induced polarization and bending curvature in graphene \cite{kalinin2008electronic}. Defect induced flexoelectricity is also observed by DFT studies \cite{Kundalwal2017,Chandratre2012} in graphene and graphene nitrids \cite{Zelisko2014anomalous}. Theoretical study \cite{kvashnin2015flexoelectricity} and DFT studies \cite{martin2017polarization} have investigated the flexoelectric effect in carbon nano structures (nanotubes, nanocones). Experiment study \cite{Brennan2017out} using piezoresponse force microscopy measured the bending flexoelectric coefficient of MoS2. Furthermore, our recently work \bh{cite prb paper} extracted the bending flexoelectric coefficients of two-dimensional materials, including graphene allotropes, nitrides, graphene analogs of group-IV elements, and the transition metal dichalcogenides (TMDCs) through MD simulation, and it reveals that the TMDCs yield the strongest flexoelectric response due to geometrical asymmetry under bending. However, the Janus TMDCs inherit a geometrical asymmetry in their nature structure, which can leads to strong flexeoelectric response and a recently DFT study \cite{dong2017large} demonstrated that Janus TMDCs have larger in-plane piezoelectric coefficients as the traditional TMDCs.\\
%\noindent In this study, we adopted the molecular dynamics simulation equipped with the charge-dipole model to investigate the bending flexoelectric coefficient of the Janus TMDCs and the mechanism behind it. The coupled model is validated with respect to the DFT calculation in terms of the in-plane piezoelectric coefficient of the Janus TMDCs, hereafter the flexoelectric coefficients of the Janus TMDCs are extracted and the underpinned mechanism is analyzed. Section 2 presents the simulation method, following by the result and discussion in section 3. The conclusion is presented in section 4.

%a linear relationship was found between induced dipole moment and bending curvature in graphene using DFT calculations~.  A theoretical analysis~\cite{kvashnin2015flexoelectricity} of flexoelectricity in carbon nanostructures (nanotubes, fullerenes and nanocones) confirmed the dependence of flexoelectric atomic dipole moments on local curvature.  Others have patterned graphene to generate strain gradients and enhance the electromechanical coupling and polarization~\cite{chandratre2012coaxing,Kundalwal2017,javvaji2018generation}. Furthermore, a recent experimental study~\cite{Brennan2017out} provided evidence that monolayer MoS$_2$ exhibits an out-of-plane flexoelectric response using the piezoresponse force microscopy.  


 %Two-dimensional materials \cite{Wang2015observattion,Song2017piezo,Zheng2017hexagonal,Zelisko2014anomalous,blonsky2015ab} including Janus TMDCs \cite{dong2017large} have exhibited outstanding electromechanical properties. However the aforementioned studies mainly focus on the piezoelectric effect of the 2D materials. In the meantime, Majdoub, et. al. \cite{majdoub2008enhanced} demonstrated that the flexoelectric effect is size-dependent, which yields a stronger electromechanical coupling at smaller scale, hence presents a great opportunity for low dimension 2D material, such as Janus TMDCs, as the next generation energy harvester thanks to their intrinsic small scale. \\
%\noindent Contrast to the extensive studies on the piezoelectric effect in 2d material, few studies on flexoelectricity in 2D materials are conducted. For instance, A Density function theory (DFT) study revealed a linear relationship between the induced polarization and bending curvature in graphene \cite{kalinin2008electronic}. Defect induced flexoelectricity is also observed by DFT studies \cite{Kundalwal2017,Chandratre2012} in graphene and graphene nitrids \cite{Zelisko2014anomalous}. Theoretical study \cite{kvashnin2015flexoelectricity} and DFT studies \cite{martin2017polarization} have investigated the flexoelectric effect in carbon nano structures (nanotubes, nanocones). Experiment study \cite{Brennan2017out} using piezoresponse force microscopy measured the bending flexoelectric coefficient of MoS2. Furthermore, our recently work \cite{zhuang2019intrinsic} extracted the bending flexoelectric coefficients of two-dimensional materials, including graphene allotropes, nitrides, graphene analogs of group-IV elements, and the transition metal dichalcogenides (TMDCs) through MD simulation, and it reveals that the TMDCs yield strongest flexoelectric response due to geometrical asymmetry under bending. However, the Janus TMDCs inherit a geometrical asymmetry in their nature structure, which can leads to strong flexeoelectric response and a recently DFT study \cite{dong2017large} demonstrated that Janus TMDCs have larger in-plane piezoelectric coefficients as the traditional TMDCs.\\
